From RDMA to RDCA: Toward High-Speed Last Mile of Data Center Networks Using Remote Direct Cache Access

In this paper, we conduct systematic measurement studies to show that the high memory bandwidth consumption of modern distributed applications can lead to a significant drop of network throughput and a large increase of tail latency in high-speed RDMA networks.We identify its root cause as the high contention of memory bandwidth between application processes and network processes. This contention leads to frequent packet drops at the NIC of receiving hosts, which triggers the congestion control mechanism of the network and eventually results in network performance degradation. To tackle this problem, we make a key observation that given the distributed storage service, the vast majority of data it receives from the network will be eventually written to high-speed storage media (e.g., SSD) by CPU. As such, we propose to bypass host memory when processing received data to completely circumvent this performance bottleneck. In particular, we design Lamda, a novel receiver cache processing system that consumes a small amount of CPU cache to process received data from the network at line rate. We implement a prototype of Lamda and evaluate its performance extensively in a Clos-based testbed. Results show that for distributed storage applications, Lamda improves network throughput by 4.7% with zero memory bandwidth consumption on storage nodes, and improves network throughput by up 17% and 45% for large block size and small size under the memory bandwidth pressure, respectively. Lamda can also be applied to latency-sensitive HPC applications, which reduces their communication latency by 35.1%.

==> congestion.tex <==
\section{Host Congestion Control}

In fact, we argue that further strengthening the NIC can completely solve the problems of the Achilles. Specifically, We can demonstrate our point of view from the following three aspects: (1) Enhance the existing packet loss retransmission mechanism to ensure performance during packet loss. (2) Enhance the queue monitoring capability of the NIC to avoid packet loss. (3) Enhance the programmability of the NIC to realize application semantic offloading for better performance.

\subsection{Selective Retransmission on NIC}

In the existing RoCE network, it performs go-back-N retransmission. When the receiver receives an out-of-order packet, it simply discards it and sends a negative acknowledgment (NACK) to the sender. When the sender sees a NACK, it retransmits all packets that were sent after the last acknowledged packet. In this way, once a problem such as packet loss occurs due to the Achilles contention, throughput will deteriorate rapidly. In the latest ConnectX-6 DX NIC, it supports selective retransmission in NIC. Although this can ensure low resource consumption, it cannot achieve high performance in scenarios with a lot of packet loss. The reason is that it can only support one PSN on the fly because of the resource limits. This means if we lost 10 packets, the receiver needs to inform the sender 10 times. Therefore, we can dynamically select the method of packet loss retransmission according to the network status. When the network packet loss is serious, enable the selective retransmission of the NIC, otherwise, enable the traditional go-back-N retransmission. This also allows us to strengthen the status of the NIC in the Achilles and packet loss recovery mechanism, so we can reduce the impact of the problems in the Achilles.

\subsection{Enable ECN on NIC}

In our data center with the lossless network, DCQCN [38] is the default congestion control algorithm that needs ECN buffer thresholds to ensure the correct operation. At an egress queue in switch, an arriving packet is ECN-marked if the queue length exceeds a threshold. This is accomplished using RED [15] functionality supported on all modern switches. ECN-marked packets arriving at the receiver indicate congestion in the network. The receiver conveys this information back to the sender. The RoCEv2 standard defines explicit Congestion Notification Packets (CNP) [38] for this purpose. From the analysis in Chapter 2, we find when there is contention in the Achilles, buffer accumulation of NIC will appear. The NIC as the entrance to the Achilles, needs more fine-grained queue control to avoid packet loss of PFC storm because of buffer overflow. The existing NIC only has a simple buffer, so some advanced operations such as buffer monitoring and buffer scheduling cannot be implemented. With the current development of network and hardware technology, the development of merchant silicon is getting better. The enhancement of hardware capabilities enables the NIC to handle more complex tasks and functions, including more complete buffer capabilities. In fact, only needing to add some most common functions of NIC can alleviate the problem of Achilles. A relatively complete buffer function is implemented on the ConnectX-6 DX NIC, which can be used to monitor the queue length and so set the ECN threshold of the queue. In other words, the traditional switch ECN marking method can be set on the NIC in the same way.

==> design_isolation.tex <==
\subsection{Cache Isolation}

we use the CAT technology (Cache Allocation Technology~\cite{cat}) to isolate a dedicated cache space of an appropriate size for the cache-resident buffer pool so that it can be resident in the cache. However, we found in our experiments that even if cache isolation is implemented, it is possible for data to be swapped out to memory, due to competition for caches such as data and instructions in \system{} process. So we slightly increase the isolated cache size appropriately to cope with this issue.

\para{Allocate dedicated cache using CAT.}
In order to avoid cache conflicts between processes, together with the memory bandwidth consumption caused by cache swapping in and swapping out, we use CAT  to allocate a dedicated cache space for \system{}. Specifically, since \system{} process and other application processes are deployed on the same node, these processes compete for the cache resource, causing the memory buffer of \system{} to be swapped out to the memory continuously. This problem is also known as the "noisy neighbor" effect~\cite{8004214}.  Therefore, we leverage the CAT technology to allocate a dedicated cache buffer for \system{} process, the size of which equals to the size of the cache-resident buffer pool. In this situation, \system{} is protected from competing with other application processes for the cache resource.

\para{A problem when using CAT.}\label{CAT}
While implementing cache isolation using CAT in our experiments, we find a bug of the CAT technology: the CAT technology can only achieve allocating restrictions but no access restrictions. Since there is competition for the cache between instruction and data, data can still be swapped out to memory even though a dedicated cache buffer is allocated using the CAT technology. What's worse, if the swapped-out data is accessed by other processes, the swapped-out data would be read into other cache groups. However, other cache groups are not dedicated to \system{}. Applications compete for cache, resulting in that part of data being frequently swapped in and out and consuming the memory bandwidth. Therefore, in order to make the cache-resident buffer pool resident in the LLC all the time, we slightly increase the size of the cache allocated to \system{}. For example, for a cache-resident buffer pool with a size of 12MB, we use CAT to allocate 15MB of cache buffer for it. Go a step further, we periodically and randomly access the data to ensure that the cache-resident buffer pool is resident in the cache.

As we can't inform the RNIC to mark ECN, we turn to decrease the ECN threshold when the usage of the cache exceeds the threshold.

==> discussion.tex <==
\section{Discussion}

% \subsection{Different Size of Used Cache}

% \subsection{Management Mechanism of Cache}

% As talked about in the section \ref{CAT}, we found a problem when suing CAT to isolate a dedicated cache for the \sysname. The root cause of this problem is that the CAT technology can only achieve allocating restrictions but no access restriction. With the development of the cache, a new cache manage mechanism is expected to be designed. Instead of isolate cache group for CPU cores, we are able to manage the cache directly, and allocate cache space for different processes.

==> motivation.tex <==
\section{Motivation}\label{sec:mot}



\subsection{Background}
\para{Direct cache access technology.} 
In classic Direct Memory Access (DMA) technology, the I/O device reads/writes data directly from/to the main memory without involving the processor. In modern computer architecture, the PCIe links support high throughput and massive connected I/O devices, consuming high bandwidth on memory. For example, a single I/O device is usually capable of from 20Gbps to 200Gbps and even 400 Gbps bandwidth[ref], and tens of I/O devices are attached to a single server. To alleviate the memory bandwidth bottleneck, Direct Cache Access (DCA) has been proposed. The current implementation of DCA technology on Intel Xeon processors, also known as Data Direct I/O (DDIO)\cite{ddio}, uses LLC as the intermediate buffer between the processor and I/O devices. Specifically, DDIO behavior can be described as follows:

\textbf{DDIO read}: I/O devices can directly read data from LLC if targeted cache lines are already resident without fetching data from memory and consuming memory read bandwidth.

\textbf{DDIO write update}: Similar to DDIO read, I/O devices can directly write data to LLC if targeted cache lines are already resident without consuming memory write bandwidth.

\textbf{DDIO write allocate}: Different from DDIO write update, DDIO write allocate is performed only when the targeted cache lines which I/O devices try to write data to are not resident. To make sure data are written to LLC instead of memory, DDIO write allocate will firstly evict victim cache lines, then write the data directly on evicted cache lines without fetching old data from memory to save memory read bandwidth. Meanwhile, the eviction may consume equivalent memory write bandwidth if memory writeback occurs.

\iffalse
\para{Memory bandwidth is a common problem.}
The development of memory lags behind that of NIC and CPU due to pin pin limitation, interface width, memory frequency, processor manufacturer and memory, and NIC manufacturer's industrial pattern of mutual separation. In the past 20 years or more, the performance of the processor has increased rapidly by about 55\% per year, while the memory performance (latency or throughput) has only increased by about 10\% per year. Over a long period of time, the unbalanced development speed has caused the current memory access speed to lag behind the processor's computing speed. The memory bottleneck has made it difficult for high-performance processors to play their due role (discuss tasks separately), that is, the memory wall problem [Scaling the Bandwidth Wall: Challenges in and Avenues for CMP Scaling]. Memory wall problems exist in storage, high-performance computing, artificial intelligence and other fields.
\fi

\subsection{Motivation}

\begin{figure*}[t]
    \centering
    \subfigure[25Gbps PFC-based network.]{
		\includegraphics[width=0.3\textwidth]{./figure/motivation/online/lossless_PFC.pdf}
		\label{fig:moti-25lossless}
	}
 \subfigure[100Gbps PFC-free network.]{
		\includegraphics[width=0.3\textwidth]{./figure/motivation/online/lossy_CNP.pdf}
		\label{fig:moti-100lossy}
	}
    \subfigure[25Gbps PFC-free network.]{
		\includegraphics[width=0.3\textwidth]{./figure/motivation/online/25G_lossy_simu_memory_bw_full.pdf}
		\label{fig:moti-25lossy}
	}
    
    \caption{Online memory bandwidth condition.}
    \label{fig:moti-online}
    
\end{figure*}


\begin{figure}[t]
\centering
	\subfigure[Network throughput.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/bw.pdf}
		\label{fig:moti-bw}
	}
	\subfigure[Network average latency.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/avg_latency.pdf}
		\label{fig:moti-avg-lat}
        }
  	\subfigure[Network P99 latency.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/p99_latency.pdf}
		\label{fig:moti-p99-lat}
	}
 	\subfigure[Average PFC and CNP.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/pfc_cnp.pdf}
		\label{fig:moti-pfc-cnp}
	}
	
	\caption{Detailed impact on the network under memory bandwidth bottleneck.}
	\label{fig:motivation-detail-net}
\end{figure}


\begin{figure}[t]
\centering
	\subfigure[PCIe back pressure.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/pcie.pdf}
		\label{fig:moti-pcie}
	}
        \subfigure[DDIO miss rate.]{
		\includegraphics[width=0.45\linewidth]{./figure/motivation/detailed_impact/ddio.pdf}
		\label{fig:moti-ddio}
	}
\caption{Detailed impact on DDIO under memory bandwidth bottleneck.}
\label{fig:motivation-detail-nic}
\end{figure}

\para{Memory bandwidth bottleneck online.}
In the 25Gb network, memory bandwidth has become a bottleneck due to the high memory access requirements from other IO devices and the repeated copy in memory. Many applications, such as distributed storage and big data processing, are memory bandwidth-sensitive applications, which almost run out of memory bandwidth. 
With the development of NICs, network throughput is growing faster and faster. The faster network speed increases the demand for memory bandwidth. For example, processing data in a 200Gbps network requires up to 400Gbps of memory bandwidth (read memory and write memory) in the worst case. The number of data transmitted on the network increases greatly. Repeated copying of these data in memory consumes a lot of memory bandwidth. What's more, after the introduction of the high-performance network, the bottleneck problem of memory bandwidth is magnified.

We collect data from an online storage cluster data to illustrate the real impact of memory bandwidth bottlenecks on the network. Specifically, our storage cluster consists of a two-tier Clos Pod with 96 storage nodes in the RDMA with the RoCEv2 network. In the lossless network (DCQCN\cite{DCQCN}+PFC (Priority Flow Control)), each server is configured with a dual port 25Gbps ConnectX-4 LX NIC, and the maximum memory bandwidth is about 60GBps under 1:1 read/write ratio. When the memory bandwidth was exhausted on lossless network shown in Figure\ref{fig:moti-25lossless}, we observed the severe burst PFC duration over 100K generated from the NIC and the average PFC duration was around 80K, which triggers PFC switch-off by watchdog and network performance degrades due to packet loss. 

In the lossy network (DCQCN), each server is configured with a dual port 100Gbps ConnectX-6 DX NIC, and the maximum memory bandwidth is about 250 GBps under 1:1 read/write ratio. When the memory bandwidth was exhausted shown in Figure\ref{fig:moti-100lossy}, we found that hundreds of Congestion Notification Packets (CNPs) were generated instantaneously due to the ECN mechanism in the ConnectX-6 DX. This mechanism can detect the watermark of the buffer inside NIC and actively send a congestion signal to the source to avoid packet loss caused by the buffer overflow. Finally, network throughput dropped by about 30\% and was unrecoverable until the memory bandwidth bottleneck disappeared.

In order to further eliminate the influence due to the network throughput and network type, we added more experiments. However, 100Gb lossless network isn't used as a production network because of the PFC storm~\cite{}, we run tests on 25Gb lossy network. When the memory bandwidth was exhausted on 25Gb lossy network shown in Figure\ref{fig:moti-moti-25lossy}, we found that up to 7217 CNPs are generated and the average number was 2268. 
% Besides, the network throughput dropped by 

In summary, the memory bandwidth bottleneck problem do exist in both 25Gb and 100Gb, lossless and lossy networks. For both lossless and lossy RoCEv2 networks, network performance is severely degraded under memory bandwidth bottleneck.

\para{Detailed analysis under the memory bandwidth bottleneck.}
We draw a conclusion from our experiment results that under the bottleneck of memory bandwidth, the DDIO write allocate operation would consume additional memory bandwidth, resulting in PCIe backpressure. Then, the packets begin to queue up in the NIC buffer and exceed the threshold, triggering the network flow control mechanism (\ie, PFC in lossless networks, and CNP in lossy networks). These flow control mechanisms ultimately lead to the increase of network latency and the decrease of throughput.

\iffalse
\para{}
On the one hand, in the RoCEv2 lossless network, PFC (Priority-based Flow Control) is used for flow control to guarantee no packet loss. When the data in the NIC buffer on the server side accumulates and exceeds the set threshold, the NIC will send a PFC pause frame to its connected upstream peer, informing the previous hop to stop sending packets. On the other hand, in RoCEv2 lossy network, DCQCN congestion control algorithm is used. When the data in the NIC buffer on the receiver side accumulates and exceeds the threshold, the message will carry the ECN congestion mark with a certain probability. If the receiver parses the message with the ECN mark, it will send the CNP congestion notification packets to notify the sender NIC to reduce the packet sending rate. What's worse, if packet loss occurs in the lossy network, the lost packets and the subsequent packets will be retransmitted due to the go-back-n protocol, which aggravates the network delay increase and throughput decrease. To sum up, when the data in the NIC buffer queues up and reaches the threshold, the flow control mechanism used by the lossless and lossy networks would reduce the number of packets sent by the sender, resulting in an increase in network latency and a decrease in throughput.

\para{}
Specifically, first, when the DDIO hit rate is low, most of the DDIO operations are write allocate. While compared with the DDIO write update operation, the DDIO write allocate operation consumes memory bandwidth when replacing the address of the original cache line into memory. That is, the leak DMA problem \todo{cite resq} happens. Second, under the memory bandwidth bottleneck, because of the extra memory bandwidth taken up by the DDIO write allocate operations, the memory bus causes PCIe backpressure, which further causes NIC backpressure. The NIC backpressure leads to data accumulation in the NIC buffer, even exceeding the threshold. To sum up, under the memory bandwidth bottleneck, the low DDIO hit rate means that most of the DDIO write allocate operations are triggered rather than the DDIO write update operations, consuming additional memory bandwidth. Then the PCIe backpressure problem happens, thus causing the amount of data in the NIC buffer to exceed the threshold.
\fi

To quantify what happened under the memory bandwidth bottleneck, we perform a fine-grained analysis.

\textbf{2 * 25 Gb-Lossless}: A dual port 25Gbps ConnectX-4 Lx NIC with PCIe 3.0 * 8. Default DDIO ways are configured as 4M.

\textbf{2 * 100 Gb-Lossy}: A dual port 100Gbps ConnectX-6 DX NIC with PCIe 4.0 * 16. Default DDIO ways are configured as 6M.

Specifically, the client sends data (4KB) with 32 QPs to the server through RDMA ib\_write\_bw by Perftest tools\cite{perftest} (modified to use multiple buffers on one QP). Moreover, we simulate applications' memory bandwidth consumption on the server through \textit{membw} from the RDT benchmark\cite{Intel_rdt}, which generates memory bandwidth by reading and writing memory of 128 MB size at a certain frequency. To monitor DDIO performance and its interaction with I/O devices, we use Intel Performance Counter Monitor (PCM) tool to count the number of PCIe write hits/misses\footnote{It will directly reflect how much DDIO write update and DDIO write allocate occur respectively}. At the same time, in order to further observe the back pressure on NIC caused by the memory bandwidth bottleneck, we use the Nvidia neohost\cite{nvidia} tool to detect detailed PCIe pressure on NICs’ side (represented as a PCIe Outbound Stalled Writes\footnote{It means the number of cycles that the PCIe unit had outbound posted write requests but could not perform the operation}).

\textbf{1. Degraded network throughput and increased latency under memory bandwidth bottleneck}. Finally, as shown in Figure \ref{fig:moti-bw}, the network throughput gradually decreases as the PCIe back pressure grows. When the IO depth is 256 (the network buffer is 32MB), the network throughput drops about 43.2\% for lossless networks and 43.1\% for lossy networks, respectively. As shown in Figure \ref{fig:moti-pfc-cnp}, in lossless network, PFC pause frame duration is generated frequently due to sustained back pressure from PCIe. In lossy network, due to the ECN control of ConnectX-6 DX NIC which can detect the watermark of the buffer inside NIC and actively send feedback to the source, packet loss is avoided in lossy network caused by overflow. As the IO depth increase, the number of CNP gradually increases and cause lower network throughput. \todo{latency}

\textbf{2. Severe back pressure from PCIe under memory bandwidth bottleneck}. Furthermore, we quantify the degree of back pressure generated by memory access from NIC under memory bandwidth bottleneck by detecting the number of PCIe outbounds stalled writes. As shown in Figure \ref{fig:moti-pcie}, a large amount of PCIe outbound stalled write is generated when DDIO write allocate is dominant (IO depth $\textgreater$ 32). The memory bandwidth consumptions on NICs’ sides result in back pressure on NICs’ PCIe under memory bandwidth bottleneck scenes firstly, before affecting network performance. The back pressure of the lossy network's PCIe is smaller than that of the lossless network because PCIe 4.0 * 16 is more redundant for 200 Gps network capability. This verifies from the side that the root cause of the network impact is the memory bandwidth bottleneck, which is different from the traditional slow receiver problem\cite{rdma_over_guo}.

\textbf{3. DDIO hit rate decreased with increasing network buffer size}. We start by detailing the specific impact of memory bandwidth bottlenecks on the network. As shown in Figure \ref{fig:moti-ddio}, with the IO depth (the number of inflight wqes) increasing, the DDIO hit rate gradually decreases. When the IO depth is 16 (the network buffer size is 2MB), the DDIO hits rate is about 99\% and 53\% for lossless and lossy networks, respectively. In this case, the network buffer is smaller than DDIO ways capacity on both configurations and no cache eviction caused by leaky DMA occurs, thus resulting in high PCIe hit rate. High PCIe hit rate leads to DDIO write update in the majority, which consumes little memory bandwidth. As IO depth increases, network buffer size also increases equivalently which overflows the DDIO ways and brings severe cache eviction.  When the IO depth is 128 (the network buffer size is about 16MB), the DDIO hits rate is about 36\% and 6\% for lossless and lossy networks, respectively. Low PCIe hit rate leads to DDIO write allocate in the majority, which requires much higher memory bandwidth to operate memory writeback when evicting cache lines for performing DDIO write allocate.

In summary, under memory bandwidth bottleneck circumstances, if frequent cache eviction caused by DDIO write allocate occurs during the DMA access from NIC to LLC,  inevitable memory access could impose PCIe back pressure on NIC, eventually leading to network performance degradation. Based on the key observation, NIC should trigger write updates as much as possible to avoid the backpressure of memory bandwidth bottleneck. 


\para{Sequence diagram}
\begin{figure*}[t]
\centering
	\subfigure[25Gbps PFC-based network throughput.]{
		\includegraphics[width=0.3\textwidth]{./figure/motivation/25G_lossless_bw.pdf}
		\label{fig:25G_lossless_bw}
	}
	\subfigure[100Gbps PFC-free network throughput.]{
		\includegraphics[width=0.3\linewidth]{./figure/motivation/100G_lossy_bw.pdf}
		\label{fig:100G_lossy_bw}
	}
	\subfigure[25Gbps PFC-free network throughput.]{
		\includegraphics[width=0.3\linewidth]{./figure/motivation/25G_lossy_bw.pdf}
		\label{fig:25G_lossy_bw}
	}
	\subfigure[25Gbps PFC-based network latency.]{
		\includegraphics[width=0.3\linewidth]{./figure/motivation/25G_lossless_lat.pdf}
		\label{fig:25G_lossless_lat}
	}
	\subfigure[100Gbps PFC-free network latency]{
		\includegraphics[width=0.3\linewidth]{./figure/motivation/100G_lossy_lat.pdf}
		\label{fig:100G_lossy_lat}
        }
  	\subfigure[25Gbps PFC-free network latency.]{
		\includegraphics[width=0.3\linewidth]{./figure/motivation/25G_lossy_lat.pdf}
		\label{fig:25G_lossy_lat}
	}
	
	\caption{Online sequence diagram.}
	\label{fig:motivation-sequence}
\end{figure*}

\wyx{As demonstrated in Figure~\ref{fig:motivation-sequence}, we recorded the time sequence diagram of network throughput and delay influenced by the memory bandwidth in three different types of networks. Figure~\ref{fig:25G_lossless_bw}, Figure~\ref{fig:100G_lossy_bw} and Figure~\ref{fig:25G_lossy_bw} show that as the memory bandwidth reaches the bottle, the network throughput drops by 14.2\%, 43.6\% and 21.3\% in 25Gbps PFC-based, 100Gbps PFC-free, and 25Gbps PFC-free networks respectively. As shown in Figure~\ref{fig:25G_lossless_lat}, Figure~\ref{fig:100G_lossy_lat} and Figure~\ref{fig:25G_lossy_lat} shows that the network average latency increases by 55.9\%,  146.0\%, and 95.3\% respectively. While the P99 latency increases by one order of magnitude in both 25Gbps PFC-based and 100Gbps PFC-free networks, and 272.3\% in 25Gbps PFC-free network.
}


==> related.tex <==
\section{Related work}

